Context-Specific Validation of Data-Driven Models

With an increasing use of data-driven models to control robotic systems, it has become important to develop a methodology for validating such models before they can be deployed to design a controller for the actual system. Specifically, it must be ensured that the controller designed for a learned model would perform as expected on the actual physical system. We propose a context-specific validation framework to quantify the quality of a learned model based on a distance measure between the closed-loop actual system and the learned model. We then propose an active sampling scheme to compute a probabilistic upper bound on this distance in a sample-efficient manner. The proposed framework validates the learned model against only those behaviors of the system that are relevant for the purpose for which we intend to use this model, and does not require any a priori knowledge of the system dynamics. Several simulations illustrate the practicality of the proposed framework for validating the models of real-world systems, and consequently, for controller synthesis.

==> notes.tex <==
Robust solutions of uncertain linear programs:
Assumes that all the uncertainties bounds are known and from an ellipsoidal set and then assumes worst case. Also the constraints are assumed to be all linear.

Robust solutions to uncertain semidefinite programs:
Here the authors consider the constraints are linear matrix inequalities with symmetric matrices.

Robust convex optimization:
Survey of the above two methods.

Robust optimization of large-scale systems:
Scenario based + linear constraints + linear cost function

New linear program performance bound for queuing network, Efficient solution algorithms for factored MDPs:
cost + constraints are linear , exploit the specific structure of the problem at hand

On constraint sampling in the linear programming approach to approximate dynamic programming:
Similar bound for sampling

LMI models :

On Avoiding Vertexization of Robustness Problems: The Approximate Feasibility Concept 
Only for those f where the robust feasibility of f(x, q) <= 0 is guaranteed if and only if f(x, q^i) <= 0 for each vertices of q^i of the l-dimensional box Q. Build an convex approximate feasibility indicator function such that and evaluate it in closed form or using Monte Carlo approaches. But to build this approximate function, we need to know the original function.

Also this is more of a feasibility approach rather than an optimization approach.

Stochastic Algorithms for Exact and Approximate Feasibility of Robust LMIs 
Learn a scalar function which projects F to the cone of positive-semidefinite matrices.  Then x is found to minimizing the expected values of this projection function over the uncertainty. 
However, we need to know what F is.
